MAQA: Evaluating Uncertainty Quantification in LLMs Regarding Data Uncertainty

Despite the massive advancements in large language models (LLMs), they still suffer from producing plausible but incorrect responses. To improve the reliability of LLMs, recent research has focused on uncertainty quantification to predict whether a response is correct or not. However, most uncertainty quantification methods have been evaluated on single-labeled questions, which removes data uncertainty: the irreducible randomness often present in user queries, which can arise from factors like multiple possible answers. This limitation may cause uncertainty quantification results to be unreliable in practical settings. In this paper, we investigate previous uncertainty quantification methods under the presence of data uncertainty. Our contributions are two-fold: 1) proposing a new Multi-Answer Question Answering dataset, MAQA, consisting of world knowledge, mathematical reasoning, and commonsense reasoning tasks to evaluate uncertainty quantification regarding data uncertainty, and 2) assessing 5 uncertainty quantification methods of diverse white- and black-box LLMs. Our findings show that previous methods relatively struggle compared to single-answer settings, though this varies depending on the task. Moreover, we observe that entropy- and consistency-based methods effectively estimate model uncertainty, even in the presence of data uncertainty. We believe these observations will guide future work on uncertainty quantification in more realistic settings.

==> tables/best_any.tex <==
\begin{table}[t]
\centering
% \small
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc|cc}
\toprule[0.1em]
\multirow{2}{*}{Model} & single & multi & best & any \\
\midrule
\midrule

\midrule
LLama-3-8b & 81.03 & 70.05 & 74.94 & 72.85 \\
Qwen-1.5-7b & 71.75 & 64.35 & 64.66 & 62.11 \\
\midrule

\bottomrule[0.1em]
\end{tabular}
}
\caption{The AUROC scores for different promptings using the Llama-3-8b model on world knowledge datasets. Priority prompting includes the additional instruction of providing answers in a way that makes the model's responses seem more probable and common.}
\label{tab:best_any}
\end{table}

==> tables/internal_priority.tex <==
\begin{table}[t]
\centering
% \small
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccc}
\toprule[0.1em]
\multirow{2}{*}{Method} & \multicolumn{3}{c}{World Knowledge NQ} & \multicolumn{3}{c}{World Knowledge HLS} \\
\cmidrule{2-7}
& precision & recall & f1 score & precision & recall & f1 score  \\
\midrule
\midrule

Max Logit & 72.85 & 65.47 & 69.74 & 59.34 & 65.69 & 67.81   \\ 
\midrule
Entropy & 72.99 & 65.96 & 70.37 & 60.07  & 66.86 & 68.00   \\
\midrule
Margin & 70.09 & 64.64 & 73.89 & 57.51 & 65.50 & 68.19   \\
\midrule
Verbalize & 67.13 & 62.05 & 64.27 & 80.56 & 69.49 & 68.75 \\
\midrule
Consistency & \textbf{88.51} & \textbf{84.51} & \textbf{88.92} & \textbf{80.79} & \textbf{90.06} & \textbf{91.24}   \\
\midrule
\bottomrule[0.1em]
\end{tabular}
}
\caption{The AUROC scores by different correctness metrics using the Llama-3-8b model on world knowledge dataset NQ and HLS.}
\label{tab:result_recall_f1}
\end{table}

==> tables/list_all_prompt.tex <==
\begin{table*}[t]
\centering
% \small
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccccccccc}
\toprule[0.1em]
\multirow{3}{*}{Method} & \multicolumn{6}{c}{World Knowledge NQ} & \multicolumn{6}{c}{World Knowledge HLS} \\
\cmidrule{2-13}
& \multicolumn{2}{c}{P} & \multicolumn{2}{c}{R} & \multicolumn{2}{c}{F1} & \multicolumn{2}{c}{P} & \multicolumn{2}{c}{R} & \multicolumn{2}{c}{F1}  \\
\cmidrule{2-13}
& V & A & V & A& V & A & V & A& V & A& V & A \\
\midrule
\midrule

Max Logit & 75.88 & 69.27 & 74.94 & 65.00 & 69.30 & 69.29  & 75.88 & 69.27 & 74.94 & 65.00 & 69.30 & 69.29 \\ 
\midrule
Entropy & 75.26 & 68.70 & 74.48 & 64.25  & 69.30 & 68.64   \\
\midrule
Margin & 73.90 & 68.43 & 74.34 & 64.25 & 69.85 & 69.95   \\
\midrule
Verbalize & 66.00 & 64.30 & 66.05 & 74.49 & 80.00 & 76.32 \\
\midrule
Consistency & 90.94 & 87.36 & 91.48 & 91.32 & 85.22 & 90.87   \\
\midrule
\bottomrule[0.1em]
\end{tabular}
}
\caption{The AUROC scores for different correctness metrics—precision (P), recall (R), and F1 score (F1)—using the Llama3-8b model on two different world knowledge datasets by different prompting; Vanilla and prompt that asks for All (A) the answers. }
\label{tab:prompting_technology}
\end{table*}

==> tables/main_result_white.tex <==
\begin{table*}[t]
\centering
\small
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccccccccccc}
\toprule[0.1em]
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{World Knowledge} & \multicolumn{3}{c}{Mathematical Reasoning} & \multicolumn{3}{c}{Commonsense Reasoning} \\
\cmidrule{3-11}
& & single & multi & all & single & multi & all & single & multi & all\\
\midrule
\midrule
% \midrule[0.01em]




\multirow{3}{*}{Qwen-7b} & logit & \textbf{73.27} & 64.68 & 67.65 & \textbf{74.36} & 64.06 & 70.70 & \textbf{59.88} & 54.05 & 57.78 & \textbf{69.17} & 60.93 & 65.38 \\
& entropy & \textbf{71.75} & 64.35 & 66.54 & \textbf{74.15} & 64.47 & 70.72 & \textbf{60.13} & 54.10 & 58.02 & \textbf{68.68} & 60.97 & 65.09 \\
& margin & \textbf{71.78} & 62.38 & 65.50 & \textbf{74.23} & 64.07 & 70.59 & \textbf{59.64} & 54.03 & 57.57 & \textbf{68.55} & 60.16 & 64.55 \\
\midrule
\multirow{3}{*}{Mistral} & logit & \textbf{54.55} & 52.47 & 52.63 & \textbf{66.17} & 60.62 & 62.34 & 36.97 & \textbf{42.88} & 40.12 & \textbf{52.56} & 51.99 & 51.70 \\
& entropy & \textbf{69.03} & 68.69 & 68.24 & \textbf{65.72} & 61.49 & 62.46 & \textbf{63.58} & 54.28 & 56.86 & \textbf{66.11} & 61.49 & 62.52 \\
& margin & \textbf{55.06} & 52.85 & 53.11 & \textbf{66.30} & 60.60 & 62.46 & 37.85 & \textbf{43.15} & 40.58 & \textbf{53.07} & 52.20 & 52.05 \\
\midrule
\multirow{3}{*}{Llama-3-8b} & logit & \textbf{81.73} & 69.64 & 74.09 & \textbf{64.85} & 59.21 & 62.48 & \textbf{58.22} & 48.72 & 49.97 & \textbf{68.27} & 59.19 & 62.18 \\
& entropy & \textbf{81.03} & 70.05 & 74.24 & \textbf{64.83} & 59.15 & 62.54 & \textbf{59.23} & 48.71 & 50.20 & \textbf{68.36} & 59.30 & 62.33 \\
& margin & \textbf{79.51} & 67.46 & 71.61 & \textbf{64.73} & 59.01 & 62.44 & \textbf{57.54} & 48.73 & 49.80 & \textbf{67.26} & 58.40 & 61.28 \\
\midrule
\multirow{3}{*}{Mixtral} & logit & 48.82 & \textbf{53.70} & 52.93 & \textbf{56.12} & 55.86 & 55.40 & 41.67 & \textbf{42.90} & 40.53 & 48.87 & \textbf{50.82} & 49.62 \\
& entropy & \textbf{72.82} & 69.40 & 71.76 & 55.83 & \textbf{60.39} & 56.70 & 58.58 & 55.48 & \textbf{59.39} & 62.41 & 61.76 & \textbf{62.62} \\
& margin & 49.14 & \textbf{53.98} & 53.17 & 56.13 & \textbf{58.54} & 56.62 & \textbf{42.62} & 42.38 & 41.24 & 49.29 & \textbf{51.63} & 50.34 \\
\midrule
\multirow{3}{*}{Llama-3-70b} & logit & \textbf{78.27} & 66.00 & 69.78 & \textbf{61.45} & 56.19 & 57.94 & 51.42 & \textbf{55.53} & 53.55 & \textbf{63.71} & 59.24 & 60.43 \\
& entropy & \textbf{79.47} & 66.45 & 70.46 & \textbf{60.87} & 55.43 & 57.28 & 51.64 & \textbf{55.46} & 53.61 & \textbf{63.99} & 59.11 & 60.45 \\
& margin & \textbf{77.38} & 65.38 & 69.09 & \textbf{60.71} & 55.40 & 57.19 & 51.16 & \textbf{55.45} & 53.40 & \textbf{63.08} & 58.74 & 59.89 \\
\midrule
\multirow{3}{*}{Qwen-72b} & logit & \textbf{74.72} & 69.67 & 71.11 & 57.25 & \textbf{66.95} & 62.26 & \textbf{74.58} & 56.36 & 62.96 & \textbf{68.85} & 64.33 & 65.44 \\
& entropy & \textbf{75.13} & 70.10 & 71.52 & 57.15 & \textbf{66.91} & 62.28 & \textbf{74.63} & 56.46 & 63.06 & \textbf{68.97} & 64.49 & 65.62 \\
& margin & \textbf{73.53} & 68.60 & 70.01 & 57.06 & \textbf{66.79} & 62.22 & \textbf{74.52} & 56.30 & 62.88 & \textbf{68.37} & 63.90 & 65.04 \\
\midrule
\multirow{3}{*}{Average} & logit & \textbf{68.56} & 62.69 & 64.70 & \textbf{63.37} & 60.48 & 61.85 & \textbf{53.79} & 50.08 & 50.82 & \textbf{61.91} & 57.75 & 59.12 \\
& entropy & \textbf{74.87} & 68.17 & 70.46 & \textbf{63.09} & 61.31 & 62.00 & \textbf{61.30} & 54.08 & 56.86 & \textbf{66.42} & 61.19 & 63.10 \\
& margin & \textbf{67.73} & 61.78 & 63.75 & \textbf{63.19} & 60.73 & 61.92 & \textbf{53.89} & 50.01 & 50.91 & \textbf{61.60} & 57.50 & 58.86 \\
\midrule
\bottomrule[0.1em]
\end{tabular}
}
% }
\caption{The AUROC scores are obtained using white-box based uncertainty quantification models on different datasets and models. A high score indicates high quantification performance. ``single'' refers to the results on a QA set with only single answers, ``multi'' refers to the \data, and ``all'' refers to the combination of these two datasets, which includes both single and multi-answer sets. \textbf{Bold} denotes the row-wise maximum AUROC for each task.}
\label{tab:main_result_white}
\vspace{-0.1in}
\end{table*}
